Masked LoGoNet: Fast and Accurate 3D Image Analysis for Medical Domain

Standard modern machine-learning-based imaging methods have faced challenges in medical applications due to the high cost of dataset construction and, thereby, the limited labeled training data available. Additionally, upon deployment, these methods are usually used to process a large volume of data on a daily basis, imposing a high maintenance cost on medical facilities. In this paper, we introduce a new neural network architecture, termed LoGoNet, with a tailored self-supervised learning (SSL) method to mitigate such challenges. LoGoNet integrates a novel feature extractor within a U-shaped architecture, leveraging Large Kernel Attention (LKA) and a dual encoding strategy to capture both long-range and short-range feature dependencies adeptly. This is in contrast to existing methods that rely on increasing network capacity to enhance feature extraction. This combination of novel techniques in our model is especially beneficial in medical image segmentation, given the difficulty of learning intricate and often irregular body organ shapes, such as the spleen. Complementary, we propose a novel SSL method tailored for 3D images to compensate for the lack of large labeled datasets. The method combines masking and contrastive learning techniques within a multi-task learning framework and is compatible with both Vision Transformer (ViT) and CNN-based models. We demonstrate the efficacy of our methods in numerous tasks across two standard datasets (i.e., BTCV and MSD). Benchmark comparisons with eight state-of-the-art models highlight LoGoNet's superior performance in both inference time and accuracy.

==> tex_files/experiment/BTCV_table_new.tex <==



\begingroup % this line and the next line reduce the table cell margins to fit in the page
\setlength{\tabcolsep}{4pt} 

\begin{table*}[]
  \centering
% \small

\begin{tabular}{c|ccccccccccccc|c}
\hline
Models                   & Spl           & RKid          & Lkid          & Gall          & Eso           & Liv           & Sto           & Aor           & IVC           & Veins         & Pan           & Rad           & Lad           & AVG           \\ \hline
UNETR                    & .912          & .940          & .938          & .693          & .690          & .954          & .754          & .891          & .830          & .703          & .734          & .660          & .577          & .790          \\
SegResNetVAE             & .941          & .938          & .933          & .670          & .718          & .955          & .745          & .892          & .848          & .695          & .783          & .633          & .528          & .791          \\
nnUNet                   & .859          & .944          & .924          & .796          & .755          & .960          & .781          & .894          & .849          & .756          & .776          & .675          & .663          & .818          \\
Attention U-Net          & .955          & .936          & .930          & .735          & .739          & .964          & .770          & .898          & .852          & .753          & .763          & .695          & .688          & .821          \\
DiNTS Instance           & .935          & .942          & .938          & .770          & .769          & .962          & .743          & .909          & .857          & .759          & .782          & .641          & .691          & .823          \\
UNet++                   & .934          & .931          & .925          & .810          & .715          & .961          & .786          & .900          & .846          & .747          & .829          & .685          & .679          & .827          \\
SwinUNETR                & .952          & .947          & .945          & .790          & .770          & .963          & .755          & .901          & .850          & .771          & .760          & .702          & .659          & .828          \\
DiNTS Search             & .937          & .934          & .930          & .788          & .770          & .960          & .774          & .904          & .866          & .751          & .813          & .670          & .711          & .831          \\ \hline
\textbf{ULKANet}         & .954          & .936          & .938          & .761          & .782          & .964          & .814          & .885          & .831          & .690          & .786          & .690          & .684          & .824          \\
\textbf{LoGoNet}         & .958          & {\ul .949}    & {\ul .947}    & .818          & .786          & .969          & .880          & .912          & .865          & .769          & .821          & .726          & .698          & .854          \\
\textbf{ULKANet + PRE}   & .954          & .940          & .933          & .836          & .794          & .966          & .853          & .899          & .854          & .760          & .823          & .703          & .734          & .850          \\
\textbf{LoGoNet + PRE}   & {\ul .961}    & .947          & .944          & .866          & .845          & {\ul .970}    & .898          & {\ul .936}    & .885          & .791          & .838          & .738          & .757          & {\ul .875}    \\ \hline
\textbf{ULKANet L}       & .948          & .938          & .933          & .832          & .789          & .967          & .832          & .888          & .862          & .744          & .784          & .720          & .690          & .841          \\
\textbf{LoGoNet L}       & .960          & .944          & .922          & .847          & .781          & \textbf{.971} & .840          & .917          & \textbf{.872} & .768          & .841          & {\ul .742}    & .710          & .855          \\
\textbf{ULKANet L + PRE} & .960          & .943          & .935          & {\ul .869}    & {\ul .863}    & {\ul .970}    & \textbf{.914} & .891          & .861          & \textbf{.806} & \textbf{.850} & .734          & {\ul .761}    & .874          \\
\textbf{LoGoNet L + PRE} & \textbf{.986} & \textbf{.963} & \textbf{.954} & \textbf{.921} & \textbf{.859} & .969          & {\ul .911}    & \textbf{.954} & {\ul .871}    & {\ul .805}    & {\ul .846}    & \textbf{.759} & \textbf{.784} & \textbf{.891} \\ \hline
\end{tabular}
  \caption{Performance of our model (in terms of Dice metric) compared to the baseline models in BTCV dataset. Spl: Spleen, RKid: Right Kidney, LKid: Left Kidney, Gall: Gallbladder, Eso: Esophagus, Liv: Liver, Sto: Stomach, Aor: Aorta, IVC: Inferior Vena Cava, Veins: Portal and Splenic Venis, Pan: Pancreas, Rad: Right Adrenal Glands, Lad: Left Adrenal Glands}
  \label{tab:BTCV_res_new}
\end{table*}

\endgroup % this line resets the table cell margins to default


==> tex_files/experiment/msd_table_new.tex <==





% \subsection{Medical Segmentation Decathlon Tasks}

% We evaluated our models with six tasks from the MSD data set. The first task is Colon Cancer, which target is \textbf{Colon Cancer Primaries}, and the challenge is heterogeneous appearance \footnote{Heterogeneous refers to a structure with dissimilar components or elements, appearing irregular or variegated. For example, a dermoid cyst has heterogeneous attenuation on CT.} The next one is \textbf{Spleen}, which of this task is large ranging foreground size. The next is \textbf{Hepatic vessels and tumor}, which challenge tubular small structures next to the heterogeneous tumor. the next one is \textbf{Pancreas Tumour}, whose target is segmenting liver and tumour; also the challenge is labeled unbalanced with large (background), medium (pancreas), and small (tumor) structures. \textbf{Lung Tumours} is the next one which challenge is  segmentation of a small target (cancer) in a large image. Also the last one is \textbf{Cardiac} which target is segment Left Atrium and chanllenge of this one is Small training dataset with large variability.

% We trained all of proposed model and based lines with 1000 epochs and table \ref{tab:MSD_res} shows the result of our experiments.


% We validated our proposed models using various tasks from the MSD dataset, conducting training for 1000 epochs. 


% Table \ref{tab:MSD_res} provides a comprehensive overview of the performance of our proposed model across six diverse tasks within the MSD dataset. Our model consistently outperforms the alternatives in the majority of these tasks, demonstrating its robustness and effectiveness in various medical image segmentation scenarios. A key contributor to our model's enhanced performance is our strategic approach to pre-training. By incorporating a comprehensive pre-training strategy, we effectively enhance the model's ability to learn meaningful representations from unlabeled data. This approach allows our model to leverage the inherent structure and patterns present in the data, leading to a notable boost in accuracy.

% The results highlight the value of our model's architecture, which integrates both local and global attention mechanisms, effectively capturing intricate spatial and contextual cues. This feature is particularly advantageous in medical image segmentation, where accurately delineating small and complex anatomical structures is crucial. Additionally, the utilization of masked SSL plays a pivotal role in improving our model's performance. The strategic inclusion of masked data within the SSL framework encourages the model to recognize long-range dependencies, leading to a more profound understanding of the underlying patterns in 3D medical images. As a result, our model achieves better accuracy, demonstrating its potential as a valuable tool in the medical imaging domain.





\begingroup % this line and the next line reduce the table cell margins to fit in the page
\setlength{\tabcolsep}{2pt} 

\begin{table}[ht]
\centering
% \small

\begin{tabular}{c|cccccc|c}
\hline
Models & Col & Spl & Hep & Pan & Lun & Car & AVG \\ \hline
UNETR & .677 & .969 & .715 & .699 & .730 & .953 & .790 \\
SegResNetVAE & .742 & .968 & .745 & .740 & .765 & .951 & .818 \\
SwinUNETR & .695 & .967 & .737 & .738 & .763 & .957 & .810 \\
nnUNet & .736 & .977 & .742 & .742 & .816 & .958 & .829 \\
Attention U-Net & - & - & - & - & - & - & - \\
UNet++ & .553 & .975 & .752 & .760 & .753 & {\ul .961} & .792 \\
DiNTS Search & .776 & \textbf{.980} & .749 & .749 & .768 & .960 & .830 \\
DiNTS Instance & .768 & {\ul .979} & .731 & .742 & .790 & \textbf{.963} & .829 \\ \hline
\textbf{ULKANet} & .773 & .976 & .730 & .768 & .788 & .942 & .830 \\
\textbf{LoGoNet} & .786 & \textbf{.980} & .757 & .798 & .802 & .951 & {\ul .846} \\
\textbf{ULKANet + PRE} & \textbf{.809} & \textbf{.980} & {\ul .776} & \textbf{.834} & {\ul .826} & .954 & \textbf{.863} \\
\textbf{LoGoNet + PRE} & {\ul .801} & \textbf{.980} & \textbf{.779} & {\ul .833} & \textbf{.828} & .958 & \textbf{.863} \\
\hline
\end{tabular}
  \caption{Performance of our model (in terms of Dice metric) compared to the baselines in MSD dataset. The baseline model ``Attention U-Net'' was not runnable on regular chipsets which each has 35 Gigabyte of memory in MSD dataset. Col: Colon Cancer Primaries, Spl: Spleen, Hep: Hepatic vessels and tumor, Pan: Pancreas Tumour,  Lun: Lung Tumours, Car: Cardiac}
  \label{tab:MSD_res}
\end{table}

\endgroup % this line resets the table cell margins to default


==> tex_files/experiment/parameter_tuning.tex <==









% \subsection{Parameter Tuning}
% \subsubsection{Multi-task Learning}
% In our proposed masked self-supervised framework, we emphasize the importance of multi-task learning as a key aspect. By leveraging multi-task learning, we incorporate various clustering algorithms into our approach, which enhances the effectiveness of our model during the relevant training phase. In this section, we aim to demonstrate the impact of the number of clustering algorithms employed for labeling purposes. The findings presented in Table \ref{tab:Ablation_res} highlight a notable trend: as the number of clusters increases, we observe improved performance for the BTCV dataset and the smaller versions of the ULKANet and LoGoNet models.

% \begin{table}[ht]
% \centering
% % \small

% \begin{tabular}{c|cccc}
% \hline


% \textbf{Model} & \textbf{N = 1} & \textbf{N = 20} & \textbf{N = 40} & \textbf{N = 80} \\ \hline
% \textbf{ULKANet + PRE} & .834 & .841 & {\ul .845} & \textbf{.850} \\
% \textbf{LoGoNet + PRE} & .860 & .866 & {\ul .868} & \textbf{.875} \\
% \hline
% \end{tabular}
%   \caption{Performance of our models at varying number of clusterers for pre-training. As the number of clusterers increases, the contribution of multi-tasking becomes more noticeable.}
%   \label{tab:Ablation_res}
% \end{table}



% By employing a greater number of clusters, we are able to capture more nuanced patterns and finer-grained information within the dataset, leading to enhanced results. This observation underscores the benefits of leveraging a diverse range of clustering algorithms within our multi-task learning approach, as it facilitates a more comprehensive and accurate labeling process. Consequently, the use of multiple clustering algorithms contributes to the improved performance of our models, as demonstrated by the experimental results on the BTCV dataset.

% It should be noted that the results presented in Table \ref{tab:Ablation_res} specifically pertain to the performance of the smaller versions of the ULKANet and LoGoNet models. This aspect highlights the scalability and generalizability of our approach, as it achieves promising results even with reduced model complexity.



